A Survey on Safety-Critical Driving Scenario Generation -- A Methodological Perspective

Autonomous driving systems have witnessed a significant development during the past years thanks to the advance in machine learning-enabled sensing and decision-making algorithms. One critical challenge for their massive deployment in the real world is their safety evaluation. Most existing driving systems are still trained and evaluated on naturalistic scenarios collected from daily life or heuristically-generated adversarial ones. However, the large population of cars, in general, leads to an extremely low collision rate, indicating that the safety-critical scenarios are rare in the collected real-world data. Thus, methods to artificially generate scenarios become crucial to measure the risk and reduce the cost. In this survey, we focus on the algorithms of safety-critical scenario generation in autonomous driving. We first provide a comprehensive taxonomy of existing algorithms by dividing them into three categories: data-driven generation, adversarial generation, and knowledge-based generation. Then, we discuss useful tools for scenario generation, including simulation platforms and packages. Finally, we extend our discussion to five main challenges of current works -- fidelity, efficiency, diversity, transferability, controllability -- and research opportunities lighted up by these challenges.

==> _survey__Safety-Critical-Scene-Generation/figs/task_tree.tex <==
\begin{tikzpicture}[
        % train/.style={fill=red!5,draw=red!50,draw},
        % both/.style={fill=red!50},
        i/.style={
            anchor=north,% south,
            align=center,
            fill=blue!20,
            rectangle,
            rounded corners,
            minimum height=8mm,
            draw=black!100,
            % very thick,
            align=center,
            text=black,
            % font=\bfseries,
            text depth = 0pt
        }
    ]
    \tikzset{execute at begin node=\strut}
    \tikzset{font=\small,
        grow=down,
        % edge from parent fork right,
        level distance=1.5cm,
        every tree node/.style={align=center,anchor=north},
        every leaf node/.style=
            {
                anchor=north,% south,
                align=center,
                fill=blue!20,
                rectangle,rounded corners,
                minimum height=10mm,
                draw=black!100,
                % thick,
                align=center,
                distance=1cm,
                text depth = -10pt
            },
        edge from parent/.style=
            {
                draw=black!100,
                thick,
                edge from parent path={(\tikzparentnode.south)
                -- +(0,-8pt)
                -| (\tikzchildnode)}
            }
    }
    
    
    \Tree [.\node[i] {Target of Generation};
    [
        .\node[i] {Algorithm Development};
        [
            .\node[i] {Not enough samples};
            {
            }
        ]
        [
            .\node[i] {Improve Robustness};
            {
            }
        ]
    ]
    [
        .\node[i] {System Evaluation};
        [
            .\node[i] {Normal Evaluation};
            {
            }
        ]
        [
            .\node[i] {Evaluate Robustness};
            {
            }
        ]
    ]
    ]
\end{tikzpicture}

==> _survey__Safety-Critical-Scene-Generation/figs/taxonomy_tree.tex <==
\begin{tikzpicture}[
        % train/.style={fill=red!5,draw=red!50,draw},
        % both/.style={fill=red!50},
        i/.style={
            anchor=north,% south,
            align=center,
            fill=blue!20,
            rectangle,rounded corners,
            minimum height=8mm,
            draw=black!100,
            % very thick,
            align=center,
            text=black,
            % font=\bfseries,
            text depth = 0pt
        }
    ]
    \tikzset{execute at begin node=\strut}
    \tikzset{font=\small,
        grow=down,
        % edge from parent fork right,
        level distance=1.5cm,
        every tree node/.style={align=center,anchor=north},
        every leaf node/.style=
            {
                anchor=north,% south,
                align=center,
                fill=blue!20,
                rectangle,rounded corners,
                minimum height=10mm,
                draw=black!100,
                % thick,
                align=center,
                distance=1cm,
                text depth = -10pt
            },
        edge from parent/.style=
            {
                draw=black!100,
                thick,
                edge from parent path={(\tikzparentnode.south)
                -- +(0,-8pt)
                -| (\tikzchildnode)}
            }
    }
    
    
    \Tree [.\node[i] {Driving \\ Scenarios};
    [
        .\node[i] {Natural \\ Scenarios};
        [
            .\node[i] {Normal Scenarios};
            [
                .\node[i] {Knowledge-based \\ Scenarios};
                {
                    \cite{mcduff2021causalcity} 
                    \cite{zhou2020smarts} 
                    \cite{cai2020summit} \\
                    \cite{fang2020augmented}
                    \cite{manivasagam2020lidarsim}
                    \cite{menzel2018scenarios}
                }
            ]
            [
                .\node[i] {Data-Driven \\ Scenarios};
                {
                    \cite{zhou2020smarts}
                    \cite{yang2020surfelgan}
                    \cite{suo2021trafficsim} \\ 
                    \cite{chen2021geosim} 
                    \cite{ehrhardt2020relate}
                    \cite{ding2018new}  \\
                    \cite{li2019aads}
                    \cite{shiroshita2020behaviorally} 
                    \cite{van2015automated}  \\
                    \cite{rocklage2017automated}
                    \cite{tan2021scenegen}
                    \cite{knies2020data} \\
                    \cite{wen2020scenario}
                    \cite{haakansson2021driving}
                    \cite{xiao2021synlidar} \\
                    \cite{wangcommonroad} 
                }
            ]
        ]
        [
            .\node[i] {Risky Scenarios};
            [
                .\node[i] {Knowledge-based \\ Scenarios};
                {
                    \cite{carlachallenge}
                }
            ]
            [
                .\node[i] {Learning-based \\ Scenarios};
                {
                    \cite{klischat2019generating}
                    \cite{althoff2018automatic}
                    \cite{wheeler2015initial} \\
                    \cite{wheeler2016factor} 
                    \cite{wulfe2018real}
                    \cite{wheeler2019critical} \\
                    \cite{o2018scalable}
                    \cite{ding2020cmts} 
                    \cite{rana2021building} \\
                    \cite{nonnengart2019crisgen}
                    \cite{klischat2020scenario}
                }
            ]
        ]
    ]
    [
        .\node[i] {Adversarial \\ Scenarios};
        [
            .\node[i] {Static Adversarial \\ Scenarios};
            {
                \cite{ding2021semantically}
                \cite{jain2019analyzing}
                \cite{tu2020physically} \\
                \cite{abdelfattah2021towards} 
                \cite{cao2019adversarial} 
                \cite{kar2019meta} \\
                \cite{devaranjan2020meta} 
                \cite{prakash2019structured} 
                \cite{khirodkar2018vadra}
            }
        ]
        [
            .\node[i] {Sequential Adversarial \\ Scenarios};
            [
                .\node[i] {Adversarial \\ Policies};
                {
                    \cite{chen2021adversarial}
                    \cite{wachi2019failure} 
                    \cite{abeysirigoonawardena2019generating} \\
                    \cite{kuutti2020training} 
                    \cite{wang2021advsim}  
                    \cite{lee2015adaptive} \\
                    \cite{koren2018adaptive}
                    \cite{koren2019efficient} 
                    \cite{koren2020adaptive} \\
                    \cite{feng2021intelligent}
                    \cite{sun2021corner} 
                    \cite{ghodsi2021generating}
                }
            ]
            [
                .\node[i] {Adversarial \\ Initial Conditions};
                {
                \cite{ding2020learning}
                \cite{ding2021multimodal}
                \cite{ruiz2018learning}
                }
            ]
        ]
    ]
    ]
\end{tikzpicture}

==> _survey__Safety-Critical-Scene-Generation/figs/taxonomy_tree_2.tex <==
\begin{tikzpicture}[
    l0/.style = {fill=gray!20, draw=black!100,thick, rounded corners, text width=30mm, align=center, anchor=north},
    l1/.style = {fill=gray!20, draw=black!100,thick, rounded corners, text width=25mm, align=center, anchor=north},
    l2/.style = {fill=gray!20, draw=black!100,thick, rounded corners, text width=30mm, align=center, anchor=north},
    l3/.style = {fill=gray!20, draw=black!100,thick, rounded corners, text width=35mm, align=center, anchor=north},
    perception/.style = {fill=color1, draw=black!100,thick, rounded corners, text width=30mm, align=center, anchor=north},
    planning/.style = {fill=color2, draw=black!100,thick, rounded corners, text width=30mm, align=center, anchor=north},
    control/.style = {fill=color3, draw=black!100,thick, rounded corners, text width=30mm, align=center, anchor=north},
    sibling distance = 42mm,
    %edge from parent fork down]
    ]
    
    \tikzset{edge from parent/.append style={thick}}
    \tikzstyle{level 1}=[sibling distance=70mm, level distance=13mm] 
    \tikzstyle{level 2}=[sibling distance=35mm, level distance=12mm] 
    \tikzstyle{level 3}=[sibling distance=35mm, level distance=10mm] 
    \tikzstyle{level 4}=[sibling distance=20mm, level distance=8mm] 
    \tikzstyle{level 5}=[sibling distance=35mm, level distance=9mm] 
    
    \node[l3] {Safety-critical \\ Scenario Generation}
        child{ 
            node[l1] {Data-driven \\ Generation \\ \textbf{(Section~\ref{sec:data})}}
            child{ 
                node[l1] {Direct \\ Sampling \\ \textbf{(Section~\ref{sec:data1})}}
                child{ 
                    node[perception] {
                    \cite{van2015automated}
                    \cite{fang2020augmented}
                    \cite{manivasagam2020lidarsim}}
                    child{
                        node[planning] {
                        \cite{scanlon2021waymo}
                        \cite{arief2018accelerated}
                        \cite{knies2020data}
                        \cite{kruber2018unsupervised}
                        \cite{kruber2019unsupervised}
                        \cite{wang2018extracting}}
                        child{
                            node[control] {N/A}
                        }
                    }
                }
            }
            child{ 
                node[l1] {Density \\ Estimation\\ \textbf{(Section~\ref{sec:data2})}}
                child{node[perception] {
                    \cite{yang2020surfelgan}  
                    \cite{chen2021geosim} 
                    \cite{ehrhardt2020relate}
                    \cite{li2019aads}
                    \cite{xiao2021synlidar}
                    \cite{kar2019meta}
                    \cite{devaranjan2020meta}
                    \cite{savkin2021unsupervised}}
                    child{
                        node[planning] {
                        \cite{ding2018new}
                        \cite{haakansson2021driving}
                        \cite{ding2020cmts}
                        \cite{huang2018synthesis}
                        \cite{guo2019modeling}
                        \cite{tan2021scenegen}
                        \cite{wen2020scenario}
                        \cite{wheeler2015initial}
                        \cite{wheeler2016factor}
                        \cite{wheeler2019critical}
                        \cite{wulfe2018real}}
                        child{
                            node[control] {
                            \cite{bojarski2016end}
                            \cite{ho2016generative}
                            \cite{chen2019deep}}
                        }
                    }
                }
            }
        }
        child{ node[l1] {Adversarial \\ Generation \\ \textbf{(Section~\ref{sec:adversarial})}}
            child{ node[l1] {Static \\ Scenarios \\ \textbf{(Section~\ref{sec:adversarial1})}}
                child{ node[perception] {
                    \cite{jain2019analyzing}
                    \cite{tu2020physically} 
                    \cite{abdelfattah2021towards} 
                    \cite{cao2019adversarial} 
                    \cite{prakash2019structured}
                    \cite{khirodkar2018vadra}
                    \cite{zhu2021adversarial}}
                    child{
                        node[planning] {N/A}
                        child{
                            node[control] {N/A}
                        }
                    }
                }
            }
            child{ node[l1] {Dynamic \\ Scenarios \\ \textbf{(Section~\ref{sec:adversarial2})}}
                child{ node[perception] {
                    \cite{ruiz2018learning}
                    \cite{o2018scalable} 
                    \cite{abeysirigoonawardena2019generating}}
                    child{
                        node[planning] {
                        \cite{ding2020learning} 
                        \cite{ding2021multimodal}
                        \cite{ghodsi2021generating}
                        \cite{wang2021advsim} 
                        \cite{nonnengart2019crisgen}
                        \cite{feng2021intelligent}
                        \cite{sun2021corner}
                        \cite{koren2018adaptive} 
                        \cite{koren2019efficient} 
                        \cite{koren2020adaptive} 
                        \cite{koren2021finding}
                        \cite{rempe2022generating}}
                        child{
                            node[control] {
                            \cite{arief2021deep}
                            \cite{arief2021certifiable}
                            \cite{chen2021adversarial}
                            \cite{wachi2019failure}
                            \cite{kuutti2020training} 
                            \cite{lee2015adaptive} }
                        }
                    }
                }
            }
        }
        child{ node[l0] {Knowledge-based \\ Generation \\ \textbf{(Section~\ref{sec:knowledge})}}
            child{ node[l1] {Pre-defined \\ Rules \\ \textbf{(Section~\ref{sec:knowledge1})}}
                child{ node[perception] {
                    \cite{cai2020summit}
                    \cite{carlachallenge}
                    \cite{li2021metadrive}
                    \cite{fremont2022scenic}
                    \cite{fremont2020formal}}
                    child{
                        node[planning] {
                        \cite{mcduff2021causalcity}
                        \cite{menzel2018scenarios}
                        \cite{bagschik2018ontology}
                        }
                        child{
                            node[control] {
                            \cite{rana2021building}
                            \cite{zhou2020smarts}}
                        }
                    }
                }
            }
            child{ node[l0] {Knowledge-guided \\ Learning \\ \textbf{(Section~\ref{sec:knowledge2})}}
                child{ node[perception] {
                    \cite{ding2021semantically}}
                    child{
                        node[planning] {
                        \cite{ding2021causalaf}
                        \cite{zhang2022adversarial}
                        \cite{cao2022robust}
                        \cite{klischat2019generating}
                        \cite{althoff2018automatic}
                        \cite{rocklage2017automated}
                        \cite{klischat2020scenario}
                        \cite{wang2021commonroad}}
                        child{
                            node[control] {
                            \cite{shiroshita2020behaviorally}}
                        }
                    }
                }
            }
        };
\end{tikzpicture}



==> _survey__Safety-Critical-Scene-Generation/tables/tab_dataset.tex <==
\begin{table*}[ht]
    \caption{Comparison of Scenario Datasets. We list existing datasets and different aspects that we are interested in. \checkmark/$\times$ in the weather column means the dataset contains/doesn't contain data under various weather conditions. BEV: bird's-eye view, FPV: first-person view. D: daytime, N: nighttime. H: highway, I: intersection, RA: roundabout, C: campus, U: urban, S: suburban, R: rural.}
    \label{tab:dataset}
    \renewcommand\arraystretch{1.2}
    \centering
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
    \hline
    \multirow{2}{*}{Dataset} & \multirow{2}{*}{\update{Year}} & \multirow{2}{*}{Real} & \multirow{2}{*}{View} & \multicolumn{4}{c|}{Data Sensor} & \multicolumn{3}{c|}{Annotation} & \multicolumn{4}{c}{Traffic Condition} \\
    \cline{5-15}
    & & & & Image & LiDAR & \update{RADAR} & Traj. & 3D & 2D & Lane & Weather & Time & Region & \update{Jam} \\
    \rowcolor{gray!30}
    \hline
    CamVid~\cite{brostow2009semantic} & 2009 & \checkmark  & FPV  & RGB & $\times$ & $\times$ & $\times$  & $\times$  & \checkmark  & \checkmark  & $\times$  & D  & U & $\times$ \\
    \hline
    KITTI~\cite{geiger2013vision} & 2013 & \checkmark  & FPV  & RGB/Stereo & \checkmark & $\times$ & $\times$  & \checkmark  & \checkmark  & \checkmark  & $\times$  & D  & U/R/H & $\times$  \\
    \hline
    \rowcolor{gray!30}
    Cyclists~\cite{li2016new} & 2016 & \checkmark  & FPV  & RGB & $\times$ & $\times$ & $\times$  & $\times$  & \checkmark  & $\times$  & $\times$  & D  & U & $\times$  \\
    \hline
    Cityscapes~\cite{cordts2016cityscapes} & 2016 & \checkmark  & FPV  & RGB/Stereo & $\times$ & $\times$ & \checkmark  & \checkmark  & \checkmark  & $\times$  & $\times$  & D  & U & \checkmark  \\
    \hline
    \rowcolor{gray!30}
    SYNTHIA~\cite{ros2016synthia} & 2016 & $\times$  & FPV  & RGB & $\times$ & $\times$ & $\times$  & \checkmark  & \checkmark  & $\times$  & \checkmark  & D/N  & U & \checkmark  \\
    \hline
    Campus~\cite{robicquet2016learning} & 2016 & \checkmark  & BEV  & RGB & $\times$ & $\times$ & \checkmark  & $\times$  & \checkmark  & \checkmark  & $\times$  & D  & C & $\times$ \\
    \hline
    \rowcolor{gray!30}
    \update{RobotCar~\cite{RobotCarDatasetIJRR}} & 2016 & \checkmark  & FPV  & RGB & \checkmark & $\times$ & \checkmark  & \checkmark  & \checkmark  & $\times$  & \checkmark  & D/N  & U & $\times$ \\
    \hline
    Mapillary~\cite{neuhold2017mapillary} & 2017 & \checkmark  & FPV  & RGB & $\times$ & $\times$ & $\times$  & $\times$  & \checkmark  & \checkmark  & \checkmark  & D/N  & U & $\times$  \\
    \hline
    \rowcolor{gray!30}
    P.F.B.~\cite{richter2017playing} & 2017 & $\times$  & FPV  & RGB & $\times$ & $\times$ & \checkmark  & \checkmark  & \checkmark  & $\times$  & \checkmark  & D/N  & U & $\times$  \\
    \hline
    BDD100K~\cite{yu2020bdd100k} & 2018 & \checkmark  & FPV  & RGB & $\times$ & $\times$ & \checkmark  & $\times$  & \checkmark  & \checkmark  & \checkmark  & D  & U/H  & $\times$ \\
    \hline
    \rowcolor{gray!30}
    HighD~\cite{krajewski2018highd} & 2018 & \checkmark  & BEV  & RGB  & $\times$ & $\times$ & \checkmark  & $\times$  & \checkmark  & $\times$  & $\times$  & D  & H & \checkmark \\
    \hline
    Udacity~\cite{udacity} & 2018 & \checkmark  & FPV  & RGB & $\times$ & $\times$ & $\times$  & $\times$  & \checkmark  & $\times$  & $\times$  & D  & U & $\times$  \\
    \hline
    \rowcolor{gray!30}
    KAIST~\cite{choi2018kaist} & 2018 & \checkmark  & FPV  & RGB/Stereo & \checkmark & $\times$ & \checkmark  & $\times$  & \checkmark  & $\times$  & $\times$  & D/N  & U & $\times$ \\
    \hline
    Argoverse~\cite{Argoverse} & 2019 & \checkmark  & FPV  & RGB/Stereo & \checkmark & $\times$ & \checkmark  & \checkmark  & $\times$  & \checkmark  & \checkmark  & D/N  & U & $\times$  \\
    \hline
    \rowcolor{gray!30}
    TRAF~\cite{chandra2019traphic} & 2019 & \checkmark  & FPV  & RGB & $\times$ & $\times$ & \checkmark  & $\times$  & \checkmark  & $\times$  & \checkmark  & D/N  & U & $\times$  \\
    \hline
    ApolloScape~\cite{huang2019apolloscape} & 2019 & \checkmark  & FPV  & RGB/Stereo & \checkmark & $\times$ & \checkmark  & \checkmark  & \checkmark  & \checkmark  & \checkmark  & D  & U & \checkmark  \\
    \hline
    \rowcolor{gray!30}
    ACFR~\cite{zyner2019acfr} & 2019 & \checkmark & BEV  & RGB & $\times$ & $\times$ & \checkmark  & $\times$  & \checkmark  & $\times$  & $\times$  & D  & RA & $\times$  \\
    \hline
    H3D~\cite{patil2019h3d} & 2019 & \checkmark  & FPV  & RGB & \checkmark & $\times$ & \checkmark  & \checkmark  & $\times$  & $\times$  & $\times$  & D  & U & \checkmark  \\
    \hline
    \rowcolor{gray!30}
    \scriptsize{INTERACTION~\cite{interactiondataset}} & 2019 & \checkmark  & BEV  & RGB & $\times$ & $\times$ & $\times$  & $\times$  & \checkmark  & \checkmark  & $\times$  & D  & I/RA & $\times$ \\
    \hline
    InD~\cite{bock2020ind} & 2020 & \checkmark  & BEV  & RGB & $\times$ & $\times$ & \checkmark  & $\times$  & \checkmark  & $\times$  & $\times$  & D  & I & $\times$ \\
    \hline
    \rowcolor{gray!30}
    RounD~\cite{krajewski2020round} & 2020 & \checkmark  & BEV  & RGB & $\times$ & $\times$ & \checkmark  & $\times$  & \checkmark  & $\times$  & $\times$  & D  & RA & $\times$ \\
    \hline
    nuScenes~\cite{caesar2020nuscenes} & 2020 & \checkmark  & FPV  & RGB & \checkmark & \checkmark & $\times$  & \checkmark  & \checkmark  & $\times$  & \checkmark  & D/N  & U & $\times$  \\
    \hline
    \rowcolor{gray!30}
    Lyft Level 5~\cite{houston2020one} & 2020 & \checkmark  & BEV  & RGB & \checkmark & \checkmark & \checkmark  & $\times$  & \checkmark  & \checkmark  & $\times$  & D  & S & $\times$ \\
    \hline
    Waymo Open~\cite{sun2020scalability} & 2020 & \checkmark  & FPV  & RGB & \checkmark & $\times$ & $\times$  & \checkmark  & \checkmark  & \checkmark  & \checkmark  & D/N  & U/S & $\times$ \\
    \hline
    \rowcolor{gray!30}
    A*3D~\cite{pham20203d} & 2020 & \checkmark  & FPV  & RGB & \checkmark & $\times$ & $\times$  & \checkmark  & \checkmark  & $\times$  & \checkmark  & D/N  & U & \checkmark  \\
    \hline
    \scriptsize{\update{RobotCar Radar~\cite{RadarRobotCarDatasetICRA2020}}} & 2020 & \checkmark  & FPV  & RGB & \checkmark & \checkmark & \checkmark  & $\times$  & $\times$  & $\times$  & \checkmark  & D/N  & U & $\times$  \\
    \hline
    \rowcolor{gray!30}
    Argoverse 2~\cite{wilson2021argoverse} & 2021 & \checkmark  & FPV  & RGB/Stereo & \checkmark & $\times$ & \checkmark  & \checkmark  & $\times$  & \checkmark  & \checkmark  & D/N  & U & $\times$  \\
    \hline
    \update{PandaSet~\cite{xiao2021pandaset}} & 2021 & \checkmark  & FPV  & RGB & \checkmark & $\times$ & \checkmark  & \checkmark  & $\times$  & $\times$  & $\times$  & D/N  & U & $\times$ \\
    \hline
    \rowcolor{gray!30}
    \update{ONCE~\cite{mao2021one}} & 2021 & \checkmark  & FPV  & RGB/Stereo & \checkmark & $\times$ & $\times$  & \checkmark  & \checkmark  & $\times$  & \checkmark  & D/N  & U & $\times$ \\
    \hline
    \end{tabular}
\end{table*}

==> _survey__Safety-Critical-Scene-Generation/tables/tab_dataset_old.tex <==
\begin{table*}[ht]
\label{tab:dataset}
    \caption{Comparison of Scenario Datasets. We list existing datasets and different aspects that we are interested in. \checkmark/$\times$ in the weather column means the dataset contains/doesn't contain data under various weather conditions. BEV: bird's-eye view, FPV: first-person view. D: daytime, N: nighttime. H: highway, I: intersection, RA: roundabout, C: campus, U: urban, S: suburban, R: rural.}
    \renewcommand\arraystretch{1.2}
    \centering
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c}
    \hline
    \multirow{2}{*}{Dataset} & \multirow{2}{*}{Real} & \multirow{2}{*}{View} & \multirow{2}{*}{\makecell[c]{RGB \\ Image}} & \multirow{2}{*}{\makecell[c]{Stereo \\ Image}} & \multirow{2}{*}{LiDAR} & \multirow{2}{*}{Trajectory} & \multicolumn{3}{c|}{Annotation} & \multicolumn{3}{c}{Traffic Condition} \\
    \cline{8-13}
    & & & & & & & 3D & 2D & Lane & Weather & Time & Environment \\
    \hline
    \rowcolor{gray!30}
    HighD~\cite{krajewski2018highd} & \checkmark  & BEV  & \checkmark  & $\times$  & $\times$  & \checkmark  & $\times$  & \checkmark  & $\times$  & $\times$  & D  & H \\
    \hline
    InD~\cite{bock2020ind} & \checkmark  & BEV  & \checkmark  & $\times$  & $\times$  & \checkmark  & $\times$  & \checkmark  & $\times$  & $\times$  & D  & I \\
    \hline
    \rowcolor{gray!30}
    RounD~\cite{krajewski2020round} & \checkmark  & BEV  & \checkmark  & $\times$  & $\times$  & \checkmark  & $\times$  & \checkmark  & $\times$  & $\times$  & D  & RA \\
    \hline
    Stanford Drone~\cite{robicquet2016learning} & \checkmark  & BEV  & \checkmark  & $\times$  & $\times$  & \checkmark  & $\times$  & \checkmark  & \checkmark  & $\times$  & D  & C \\
    \hline
    \rowcolor{gray!30}
    Five Roundabouts~\cite{zyner2019acfr} & \checkmark  & BEV  & \checkmark  & $\times$  & $\times$  & \checkmark  & $\times$  & \checkmark  & $\times$  & $\times$  & D  & RA  \\
    \hline
    INTERACTION~\cite{interactiondataset} & \checkmark  & BEV  & \checkmark  & $\times$  & $\times$  & $\times$  & $\times$  & \checkmark  & \checkmark  & $\times$  & D  & I, RA \\
    \hline
    \rowcolor{gray!30}
    Lyft Level 5~\cite{houston2020one} & \checkmark  & BEV  & \checkmark  & $\times$  & \checkmark  & \checkmark  & $\times$  & \checkmark  & \checkmark  & $\times$  & D  & S \\
    \hline
    Cyclists~\cite{li2016new} & \checkmark  & FPV  & \checkmark  & $\times$  & $\times$  & $\times$  & $\times$  & \checkmark  & $\times$  & $\times$  & D  & U  \\
    \hline
    \rowcolor{gray!30}
    Udacity~\cite{udacity} & \checkmark  & FPV  & \checkmark  & $\times$  & $\times$  & $\times$  & $\times$  & \checkmark  & $\times$  & $\times$  & D  & U  \\
    \hline
    TRAF~\cite{chandra2019traphic} & \checkmark  & FPV  & \checkmark  & $\times$  & $\times$  & \checkmark  & $\times$  & \checkmark  & $\times$  & \checkmark  & D/N  & U  \\
    \hline
    \rowcolor{gray!30}
    Argoverse~\cite{Argoverse} & \checkmark  & FPV  & \checkmark  & \checkmark  & \checkmark  & \checkmark  & \checkmark  & $\times$  & \checkmark  & \checkmark  & D/N  & U  \\
    \hline
    Argoverse 2~\cite{wilson2021argoverse} & \checkmark  & FPV  & \checkmark  & \checkmark  & \checkmark  & \checkmark  & \checkmark  & $\times$  & \checkmark  & \checkmark  & D/N  & U  \\
    \hline
    \rowcolor{gray!30}
    ApolloScape~\cite{huang2019apolloscape} & \checkmark  & FPV  & \checkmark  & \checkmark  & \checkmark  & \checkmark  & \checkmark  & \checkmark  & \checkmark  & \checkmark  & D  & U  \\
    \hline
    CamVid~\cite{brostow2009semantic} & \checkmark  & FPV  & \checkmark  & $\times$  & $\times$  & $\times$  & $\times$  & \checkmark  & \checkmark  & $\times$  & D  & U \\
    \hline
    \rowcolor{gray!30}
    KITTI~\cite{geiger2013vision} & \checkmark  & FPV  & \checkmark  & \checkmark  & \checkmark  & $\times$  & \checkmark  & \checkmark  & \checkmark  & $\times$  & D  & U, R, H  \\
    \hline
    Cityscapes~\cite{cordts2016cityscapes} & \checkmark  & FPV  & \checkmark  & \checkmark  & $\times$  & \checkmark  & \checkmark  & \checkmark  & $\times$  & $\times$  & D  & U  \\
    \hline
    \rowcolor{gray!30}
    Mapillary~\cite{neuhold2017mapillary} & \checkmark  & FPV  & \checkmark  & $\times$  & $\times$  & $\times$  & $\times$  & \checkmark  & \checkmark  & \checkmark  & D/N  & U  \\
    \hline
    BDD100K~\cite{yu2018bdd100k} & \checkmark  & FPV  & \checkmark  & $\times$  & $\times$  & \checkmark  & $\times$  & \checkmark  & \checkmark  & \checkmark  & D  & U, H  \\
    \hline
    \rowcolor{gray!30}
    nuScenes~\cite{caesar2020nuscenes} & \checkmark  & FPV  & \checkmark  & $\times$  & \checkmark  & $\times$  & \checkmark  & \checkmark  & $\times$  & \checkmark  & D/N  & U  \\
    \hline
    KAIST~\cite{choi2018kaist} & \checkmark  & FPV  & \checkmark  & \checkmark  & \checkmark  & \checkmark  & $\times$  & \checkmark  & $\times$  & $\times$  & D/N  & U \\
    \hline
    \rowcolor{gray!30}
    H3D~\cite{patil2019h3d} & \checkmark  & FPV  & \checkmark  & $\times$  & \checkmark  & \checkmark  & \checkmark  & $\times$  & $\times$  & $\times$  & D  & U  \\
    \hline
    Waymo Open~\cite{sun2020scalability} & \checkmark  & FPV  & \checkmark  & $\times$  & \checkmark  & $\times$  & \checkmark  & \checkmark  & \checkmark  & \checkmark  & D/N  & U, S \\
    \hline
    \rowcolor{gray!30}
    A*3D~\cite{pham20203d} & \checkmark  & FPV  & \checkmark  & $\times$  & \checkmark  & $\times$  & \checkmark  & \checkmark  & $\times$  & \checkmark  & D/N  & U  \\
    \hline
    P.F.B.~\cite{richter2017playing} & $\times$  & FPV  & \checkmark  & $\times$  & $\times$  & \checkmark  & \checkmark  & \checkmark  & $\times$  & \checkmark  & D/N  & U  \\
    \hline
    \rowcolor{gray!30}
    SYNTHIA~\cite{ros2016synthia} & $\times$  & FPV  & \checkmark  & $\times$  & $\times$  & $\times$  & \checkmark  & \checkmark  & $\times$  & \checkmark  & D/N  & U  \\
    \hline
    Deepdrive~\cite{deepdrivedata} & $\times$  & FPV  & \checkmark  & $\times$  & \checkmark  & \checkmark  & $\times$  & $\times$  & $\times$  & $\times$  & D/N  & U  \\
    \hline
    \end{tabular}
\end{table*}

==> _survey__Safety-Critical-Scene-Generation/tables/tab_platform.tex <==
\begin{table*}[ht]
    \caption{Comparison of Traffic Simulation}
    \label{tab:simulator}
    \renewcommand\arraystretch{1.2}
    \centering
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
    \hline
    \multirow{2}{*}{Simulator}  &  \multirow{2}{*}{\update{Year}}  & \multirow{2}{*}{\makecell[c]{Open \\ Source}} & \multirow{2}{*}{\makecell[c]{Realistic \\ Perception}} & \multirow{2}{*}{\makecell[c]{Customized \\ Scenario}} & \multirow{2}{*}{\makecell[c]{Back-end}} & \multicolumn{2}{c|}{Map Source}  & \multicolumn{3}{c}{API Support} \\
    \cline{7-11}
    & & & & & & Real World  & Human Design  & Python  & C++  & ROS  \\
    \hline
    \rowcolor{gray!30}
    TORCE~\cite{wymann2000torcs}                 & 2000 & \checkmark  & \checkmark  & $\times$  & None  & $\times$  & \checkmark  & $\times$  & \checkmark  & $\times$ \\
    \hline
    Webots~\cite{Webots04}                       & 2004 & \checkmark  & \checkmark  & \checkmark  & ODE  & \checkmark  & \checkmark  & \checkmark  & \checkmark  & \checkmark \\  % etc.
    \hline
    \rowcolor{gray!30}
    CarRacing~\cite{CarRacing}                   & 2016 & \checkmark  & $\times$  & $\times$  & None  & $\times$  & \checkmark  & \checkmark  & $\times$  & $\times$ \\
    \hline
    CARLA~\cite{dosovitskiy2017carla}            & 2017 & \checkmark  & \checkmark  & \checkmark  & UE4  & $\times$  & \checkmark  & \checkmark  & \checkmark  & \checkmark  \\
    \hline
    \rowcolor{gray!30}
    SimMobilityST~\cite{azevedo2017simmobility}  & 2017 & \checkmark  & $\times$  & \checkmark  & None  & $\times$  & \checkmark  & \checkmark  & $\times$  & $\times$ \\
    \hline
    GTA-V~\cite{richter2017playing}              & 2017 & $\times$  & \checkmark  & \checkmark  & RAGE  & $\times$  & $\times$  & $\times$  & $\times$  & $\times$ \\
    \hline
    \rowcolor{gray!30}
    highway-env~\cite{highway-env}               & 2018 & \checkmark  & $\times$  & \checkmark  & None  & $\times$  & \checkmark  & \checkmark  & $\times$  & $\times$ \\
    \hline
    Deepdrive~\cite{deepdrive}                   & 2018 & \checkmark  & \checkmark  & \checkmark  & UE4  & $\times$  & \checkmark  & \checkmark  & \checkmark  & $\times$ \\
    \hline
    \rowcolor{gray!30}
    esmini~\cite{esmini}                         & 2018 & \checkmark  & \checkmark  & \checkmark  & Unity  & $\times$  & \checkmark  & \checkmark  & \checkmark  & $\times$ \\
    \hline
    AutonoViSim~\cite{best2018autonovi}          & 2018 & $\times$  & \checkmark  & \checkmark  & PhysX  & $\times$  & \checkmark  & $\times$  & $\times$  & $\times$ \\
    \hline
    \rowcolor{gray!30}
    AirSim~\cite{shah2018airsim}                 & 2018 & \checkmark  & \checkmark  & \checkmark  & UE4  & $\times$  & \checkmark  & \checkmark  & \checkmark  & \checkmark \\
    \hline
    SUMO~\cite{lopez2018microscopic}             & 2018 & \checkmark  & $\times$  & \checkmark  & None  & \checkmark  & \checkmark  & \checkmark  & \checkmark  & $\times$ \\  % etc.
    \hline
    \rowcolor{gray!30}
    Apollo~\cite{apollosimulation}               & 2018 & \checkmark  & $\times$  & \checkmark  & Unity  & $\times$  & \checkmark  & \checkmark  & \checkmark  & $\times$ \\
    \hline
    Sim4CV~\cite{muller2018sim4cv}               & 2018 & \checkmark  & \checkmark  & \checkmark  & UE4  & $\times$  & \checkmark  &  \checkmark  & \checkmark  & $\times$ \\  % Matlab
    \hline
    \rowcolor{gray!30}
    SUMMIT~\cite{cai2020summit}                  & 2020 & \checkmark  & \checkmark  & $\times$  & UE4  & \checkmark  & \checkmark  & \checkmark  & $\times$  & \checkmark \\
    \hline
    MultiCarRacing~\cite{SSG2020}                & 2020 & \checkmark  & $\times$  & $\times$  & None  & $\times$  & \checkmark  & \checkmark  & $\times$  & $\times$ \\
    \hline
    \rowcolor{gray!30}
    SMARTS~\cite{zhou2020smarts}                 & 2020 & \checkmark  & $\times$  & \checkmark  & None  & $\times$  & \checkmark  & \checkmark  & $\times$  & $\times$ \\
    \hline
    LGSVL~\cite{rong2020lgsvl}                   & 2020 & \checkmark  & \checkmark  & \checkmark  & Unity  & \checkmark  & \checkmark  & \checkmark  & $\times$  & \checkmark \\
    \hline
    \rowcolor{gray!30}
    CausalCity~\cite{mcduff2021causalcity}       & 2021 & \checkmark  & \checkmark  & \checkmark  & UE4  & $\times$  & \checkmark  & \checkmark  & $\times$  & $\times$ \\
    \hline
    MetaDrive~\cite{li2021metadrive}             & 2021 & \checkmark  & \checkmark  & \checkmark  & Panda3D  & \checkmark  & \checkmark  & \checkmark  & $\times$  & $\times$ \\
    \hline
    \rowcolor{gray!30}
    L2R~\cite{herman2021learn}                   & 2021 & \checkmark  & \checkmark  & \checkmark  & UE4  & \checkmark  & \checkmark  & \checkmark  & $\times$  & $\times$ \\
    \hline
    AutoDRIVE~\cite{samak2021autodrive}          & 2021 & \checkmark  & \checkmark  & \checkmark  & Unity  & $\times$  & \checkmark  & \checkmark  & \checkmark  & \checkmark \\
    \hline
    \end{tabular}
\end{table*}

==> figs/task_tree.tex <==
\begin{tikzpicture}[
        % train/.style={fill=red!5,draw=red!50,draw},
        % both/.style={fill=red!50},
        i/.style={
            anchor=north,% south,
            align=center,
            fill=blue!20,
            rectangle,
            rounded corners,
            minimum height=8mm,
            draw=black!100,
            % very thick,
            align=center,
            text=black,
            % font=\bfseries,
            text depth = 0pt
        }
    ]
    \tikzset{execute at begin node=\strut}
    \tikzset{font=\small,
        grow=down,
        % edge from parent fork right,
        level distance=1.5cm,
        every tree node/.style={align=center,anchor=north},
        every leaf node/.style=
            {
                anchor=north,% south,
                align=center,
                fill=blue!20,
                rectangle,rounded corners,
                minimum height=10mm,
                draw=black!100,
                % thick,
                align=center,
                distance=1cm,
                text depth = -10pt
            },
        edge from parent/.style=
            {
                draw=black!100,
                thick,
                edge from parent path={(\tikzparentnode.south)
                -- +(0,-8pt)
                -| (\tikzchildnode)}
            }
    }
    
    
    \Tree [.\node[i] {Target of Generation};
    [
        .\node[i] {Algorithm Development};
        [
            .\node[i] {Not enough samples};
            {
            }
        ]
        [
            .\node[i] {Improve Robustness};
            {
            }
        ]
    ]
    [
        .\node[i] {System Evaluation};
        [
            .\node[i] {Normal Evaluation};
            {
            }
        ]
        [
            .\node[i] {Evaluate Robustness};
            {
            }
        ]
    ]
    ]
\end{tikzpicture}

==> figs/taxonomy_tree.tex <==
\begin{tikzpicture}[
        % train/.style={fill=red!5,draw=red!50,draw},
        % both/.style={fill=red!50},
        i/.style={
            anchor=north,% south,
            align=center,
            fill=blue!20,
            rectangle,rounded corners,
            minimum height=8mm,
            draw=black!100,
            % very thick,
            align=center,
            text=black,
            % font=\bfseries,
            text depth = 0pt
        }
    ]
    \tikzset{execute at begin node=\strut}
    \tikzset{font=\small,
        grow=down,
        % edge from parent fork right,
        level distance=1.5cm,
        every tree node/.style={align=center,anchor=north},
        every leaf node/.style=
            {
                anchor=north,% south,
                align=center,
                fill=blue!20,
                rectangle,rounded corners,
                minimum height=10mm,
                draw=black!100,
                % thick,
                align=center,
                distance=1cm,
                text depth = -10pt
            },
        edge from parent/.style=
            {
                draw=black!100,
                thick,
                edge from parent path={(\tikzparentnode.south)
                -- +(0,-8pt)
                -| (\tikzchildnode)}
            }
    }
    
    
    \Tree [.\node[i] {Driving \\ Scenarios};
    [
        .\node[i] {Natural \\ Scenarios};
        [
            .\node[i] {Normal Scenarios};
            [
                .\node[i] {Knowledge-based \\ Scenarios};
                {
                    \cite{mcduff2021causalcity} 
                    \cite{zhou2020smarts} 
                    \cite{cai2020summit} \\
                    \cite{fang2020augmented}
                    \cite{manivasagam2020lidarsim}
                    \cite{menzel2018scenarios}
                }
            ]
            [
                .\node[i] {Data-Driven \\ Scenarios};
                {
                    \cite{zhou2020smarts}
                    \cite{yang2020surfelgan}
                    \cite{suo2021trafficsim} \\ 
                    \cite{chen2021geosim} 
                    \cite{ehrhardt2020relate}
                    \cite{ding2018new}  \\
                    \cite{li2019aads}
                    \cite{shiroshita2020behaviorally} 
                    \cite{van2015automated}  \\
                    \cite{rocklage2017automated}
                    \cite{tan2021scenegen}
                    \cite{knies2020data} \\
                    \cite{wen2020scenario}
                    \cite{haakansson2021driving}
                    \cite{xiao2021synlidar} \\
                    \cite{wangcommonroad} 
                }
            ]
        ]
        [
            .\node[i] {Risky Scenarios};
            [
                .\node[i] {Knowledge-based \\ Scenarios};
                {
                    \cite{carlachallenge}
                }
            ]
            [
                .\node[i] {Learning-based \\ Scenarios};
                {
                    \cite{klischat2019generating}
                    \cite{althoff2018automatic}
                    \cite{wheeler2015initial} \\
                    \cite{wheeler2016factor} 
                    \cite{wulfe2018real}
                    \cite{wheeler2019critical} \\
                    \cite{o2018scalable}
                    \cite{ding2020cmts} 
                    \cite{rana2021building} \\
                    \cite{nonnengart2019crisgen}
                    \cite{klischat2020scenario}
                }
            ]
        ]
    ]
    [
        .\node[i] {Adversarial \\ Scenarios};
        [
            .\node[i] {Static Adversarial \\ Scenarios};
            {
                \cite{ding2021semantically}
                \cite{jain2019analyzing}
                \cite{tu2020physically} \\
                \cite{abdelfattah2021towards} 
                \cite{cao2019adversarial} 
                \cite{kar2019meta} \\
                \cite{devaranjan2020meta} 
                \cite{prakash2019structured} 
                \cite{khirodkar2018vadra}
            }
        ]
        [
            .\node[i] {Sequential Adversarial \\ Scenarios};
            [
                .\node[i] {Adversarial \\ Policies};
                {
                    \cite{chen2021adversarial}
                    \cite{wachi2019failure} 
                    \cite{abeysirigoonawardena2019generating} \\
                    \cite{kuutti2020training} 
                    \cite{wang2021advsim}  
                    \cite{lee2015adaptive} \\
                    \cite{koren2018adaptive}
                    \cite{koren2019efficient} 
                    \cite{koren2020adaptive} \\
                    \cite{feng2021intelligent}
                    \cite{sun2021corner} 
                    \cite{ghodsi2021generating}
                }
            ]
            [
                .\node[i] {Adversarial \\ Initial Conditions};
                {
                \cite{ding2020learning}
                \cite{ding2021multimodal}
                \cite{ruiz2018learning}
                }
            ]
        ]
    ]
    ]
\end{tikzpicture}

==> tables/tab_dataset_old.tex <==
\begin{table*}[ht]
\label{tab:dataset}
    \caption{Comparison of Scenario Datasets. We list existing datasets and different aspects that we are interested in. \checkmark/$\times$ in the weather column means the dataset contains/doesn't contain data under various weather conditions. BEV: bird's-eye view, FPV: first-person view. D: daytime, N: nighttime. H: highway, I: intersection, RA: roundabout, C: campus, U: urban, S: suburban, R: rural.}
    \renewcommand\arraystretch{1.2}
    \centering
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c}
    \hline
    \multirow{2}{*}{Dataset} & \multirow{2}{*}{Real} & \multirow{2}{*}{View} & \multirow{2}{*}{\makecell[c]{RGB \\ Image}} & \multirow{2}{*}{\makecell[c]{Stereo \\ Image}} & \multirow{2}{*}{LiDAR} & \multirow{2}{*}{Trajectory} & \multicolumn{3}{c|}{Annotation} & \multicolumn{3}{c}{Traffic Condition} \\
    \cline{8-13}
    & & & & & & & 3D & 2D & Lane & Weather & Time & Environment \\
    \hline
    \rowcolor{gray!30}
    HighD~\cite{krajewski2018highd} & \checkmark  & BEV  & \checkmark  & $\times$  & $\times$  & \checkmark  & $\times$  & \checkmark  & $\times$  & $\times$  & D  & H \\
    \hline
    InD~\cite{bock2020ind} & \checkmark  & BEV  & \checkmark  & $\times$  & $\times$  & \checkmark  & $\times$  & \checkmark  & $\times$  & $\times$  & D  & I \\
    \hline
    \rowcolor{gray!30}
    RounD~\cite{krajewski2020round} & \checkmark  & BEV  & \checkmark  & $\times$  & $\times$  & \checkmark  & $\times$  & \checkmark  & $\times$  & $\times$  & D  & RA \\
    \hline
    Stanford Drone~\cite{robicquet2016learning} & \checkmark  & BEV  & \checkmark  & $\times$  & $\times$  & \checkmark  & $\times$  & \checkmark  & \checkmark  & $\times$  & D  & C \\
    \hline
    \rowcolor{gray!30}
    Five Roundabouts~\cite{zyner2019acfr} & \checkmark  & BEV  & \checkmark  & $\times$  & $\times$  & \checkmark  & $\times$  & \checkmark  & $\times$  & $\times$  & D  & RA  \\
    \hline
    INTERACTION~\cite{interactiondataset} & \checkmark  & BEV  & \checkmark  & $\times$  & $\times$  & $\times$  & $\times$  & \checkmark  & \checkmark  & $\times$  & D  & I, RA \\
    \hline
    \rowcolor{gray!30}
    Lyft Level 5~\cite{houston2020one} & \checkmark  & BEV  & \checkmark  & $\times$  & \checkmark  & \checkmark  & $\times$  & \checkmark  & \checkmark  & $\times$  & D  & S \\
    \hline
    Cyclists~\cite{li2016new} & \checkmark  & FPV  & \checkmark  & $\times$  & $\times$  & $\times$  & $\times$  & \checkmark  & $\times$  & $\times$  & D  & U  \\
    \hline
    \rowcolor{gray!30}
    Udacity~\cite{udacity} & \checkmark  & FPV  & \checkmark  & $\times$  & $\times$  & $\times$  & $\times$  & \checkmark  & $\times$  & $\times$  & D  & U  \\
    \hline
    TRAF~\cite{chandra2019traphic} & \checkmark  & FPV  & \checkmark  & $\times$  & $\times$  & \checkmark  & $\times$  & \checkmark  & $\times$  & \checkmark  & D/N  & U  \\
    \hline
    \rowcolor{gray!30}
    Argoverse~\cite{Argoverse} & \checkmark  & FPV  & \checkmark  & \checkmark  & \checkmark  & \checkmark  & \checkmark  & $\times$  & \checkmark  & \checkmark  & D/N  & U  \\
    \hline
    Argoverse 2~\cite{wilson2021argoverse} & \checkmark  & FPV  & \checkmark  & \checkmark  & \checkmark  & \checkmark  & \checkmark  & $\times$  & \checkmark  & \checkmark  & D/N  & U  \\
    \hline
    \rowcolor{gray!30}
    ApolloScape~\cite{huang2019apolloscape} & \checkmark  & FPV  & \checkmark  & \checkmark  & \checkmark  & \checkmark  & \checkmark  & \checkmark  & \checkmark  & \checkmark  & D  & U  \\
    \hline
    CamVid~\cite{brostow2009semantic} & \checkmark  & FPV  & \checkmark  & $\times$  & $\times$  & $\times$  & $\times$  & \checkmark  & \checkmark  & $\times$  & D  & U \\
    \hline
    \rowcolor{gray!30}
    KITTI~\cite{geiger2013vision} & \checkmark  & FPV  & \checkmark  & \checkmark  & \checkmark  & $\times$  & \checkmark  & \checkmark  & \checkmark  & $\times$  & D  & U, R, H  \\
    \hline
    Cityscapes~\cite{cordts2016cityscapes} & \checkmark  & FPV  & \checkmark  & \checkmark  & $\times$  & \checkmark  & \checkmark  & \checkmark  & $\times$  & $\times$  & D  & U  \\
    \hline
    \rowcolor{gray!30}
    Mapillary~\cite{neuhold2017mapillary} & \checkmark  & FPV  & \checkmark  & $\times$  & $\times$  & $\times$  & $\times$  & \checkmark  & \checkmark  & \checkmark  & D/N  & U  \\
    \hline
    BDD100K~\cite{yu2018bdd100k} & \checkmark  & FPV  & \checkmark  & $\times$  & $\times$  & \checkmark  & $\times$  & \checkmark  & \checkmark  & \checkmark  & D  & U, H  \\
    \hline
    \rowcolor{gray!30}
    nuScenes~\cite{caesar2020nuscenes} & \checkmark  & FPV  & \checkmark  & $\times$  & \checkmark  & $\times$  & \checkmark  & \checkmark  & $\times$  & \checkmark  & D/N  & U  \\
    \hline
    KAIST~\cite{choi2018kaist} & \checkmark  & FPV  & \checkmark  & \checkmark  & \checkmark  & \checkmark  & $\times$  & \checkmark  & $\times$  & $\times$  & D/N  & U \\
    \hline
    \rowcolor{gray!30}
    H3D~\cite{patil2019h3d} & \checkmark  & FPV  & \checkmark  & $\times$  & \checkmark  & \checkmark  & \checkmark  & $\times$  & $\times$  & $\times$  & D  & U  \\
    \hline
    Waymo Open~\cite{sun2020scalability} & \checkmark  & FPV  & \checkmark  & $\times$  & \checkmark  & $\times$  & \checkmark  & \checkmark  & \checkmark  & \checkmark  & D/N  & U, S \\
    \hline
    \rowcolor{gray!30}
    A*3D~\cite{pham20203d} & \checkmark  & FPV  & \checkmark  & $\times$  & \checkmark  & $\times$  & \checkmark  & \checkmark  & $\times$  & \checkmark  & D/N  & U  \\
    \hline
    P.F.B.~\cite{richter2017playing} & $\times$  & FPV  & \checkmark  & $\times$  & $\times$  & \checkmark  & \checkmark  & \checkmark  & $\times$  & \checkmark  & D/N  & U  \\
    \hline
    \rowcolor{gray!30}
    SYNTHIA~\cite{ros2016synthia} & $\times$  & FPV  & \checkmark  & $\times$  & $\times$  & $\times$  & \checkmark  & \checkmark  & $\times$  & \checkmark  & D/N  & U  \\
    \hline
    Deepdrive~\cite{deepdrivedata} & $\times$  & FPV  & \checkmark  & $\times$  & \checkmark  & \checkmark  & $\times$  & $\times$  & $\times$  & $\times$  & D/N  & U  \\
    \hline
    \end{tabular}
\end{table*}
